Adapt then Unlearn: Exploring Parameter Space Semantics for Unlearning in Generative Adversarial Networks

Owing to the growing concerns about privacy and regulatory compliance, it is desirable to regulate the output of generative models. To that end, the objective of this work is to prevent the generation of outputs containing undesired features from a pre-trained Generative Adversarial Network (GAN) where the underlying training data set is inaccessible. Our approach is inspired by the observation that the parameter space of GANs exhibits meaningful directions that can be leveraged to suppress specific undesired features. However, such directions usually result in the degradation of the quality of generated samples. Our proposed two-stage method, known as 'Adapt-then-Unlearn,' excels at unlearning such undesirable features while also maintaining the quality of generated samples. In the initial stage, we adapt a pre-trained GAN on a set of negative samples (containing undesired features) provided by the user. Subsequently, we train the original pre-trained GAN using positive samples, along with a repulsion regularizer. This regularizer encourages the learned model parameters to move away from the parameters of the adapted model (first stage) while not degrading the generation quality. We provide theoretical insights into the proposed method. To the best of our knowledge, our approach stands as the first method addressing unlearning within the realm of high-fidelity GANs (such as StyleGAN). We validate the effectiveness of our method through comprehensive experiments, encompassing both class-level unlearning on the MNIST and AFHQ dataset and feature-level unlearning tasks on the CelebA-HQ dataset. Our code and implementation is available at: https://github.com/atriguha/Adapt_Unlearn.

==> unlearnin-results-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table*}[!ht]
% \centering
% \caption{PUL ($\uparrow$), FID ($\downarrow$) and Ret-FID ($\downarrow$) after unlearning MNIST classes and CelebA-HQ features. }
% \label{tab:comb-results}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|rrrrrrrrr|rrrrrrrrrrrr}
% \toprule
% \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Method}}} & \multicolumn{9}{c|}{\textbf{MNIST}}                                                                                                                                                                                                                                                                                                     & \multicolumn{12}{c}{\textbf{CelebA-HQ}}                                                                                                                                                                                                                                                                                                                                                                                                              \\ \cline{2-22} 
% \multicolumn{1}{c|}{}                                 & \multicolumn{3}{c|}{\textbf{Class - 1}}                                                                     & \multicolumn{3}{c|}{\textbf{Class - 4}}                                                                     & \multicolumn{3}{c|}{\textbf{Class - 8}}                                                                     & \multicolumn{3}{c|}{\textbf{Bangs}}                                                                         & \multicolumn{3}{c|}{\textbf{Hat}}                                                                           & \multicolumn{3}{c|}{\textbf{Bald}}                                                                          & \multicolumn{3}{c}{\textbf{Eyeglasses}}                                                                    \\
% \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c}{\textbf{PUL}} & \multicolumn{1}{c}{\textbf{FID}} & \multicolumn{1}{c|}{\textbf{Ret-FID}} & \multicolumn{1}{c}{\textbf{PUL}} & \multicolumn{1}{c}{\textbf{FID}} & \multicolumn{1}{c|}{\textbf{Ret-FID}} & \multicolumn{1}{c}{\textbf{PUL}} & \multicolumn{1}{c}{\textbf{FID}} & \multicolumn{1}{c|}{\textbf{Ret-FID}} & \multicolumn{1}{c}{\textbf{PUL}} & \multicolumn{1}{c}{\textbf{FID}} & \multicolumn{1}{c|}{\textbf{Ret-FID}} & \multicolumn{1}{c}{\textbf{PUL}} & \multicolumn{1}{c}{\textbf{FID}} & \multicolumn{1}{c|}{\textbf{Ret-FID}} & \multicolumn{1}{c}{\textbf{PUL}} & \multicolumn{1}{c}{\textbf{FID}} & \multicolumn{1}{c|}{\textbf{Ret-FID}} & \multicolumn{1}{c}{\textbf{PUL}} & \multicolumn{1}{c}{\textbf{FID}} & \multicolumn{1}{c}{\textbf{Ret-FID}} \\ \midrule
% \textbf{Retraining}                                   & $98.80\pm 0.09$                  & $4.94\pm 0.04$                   & \multicolumn{1}{r|}{N/A}              & $98.58\pm 0.28$                  & $5.24\pm 0.09$                   & \multicolumn{1}{r|}{N/A}              & $99.72\pm 0.01$                  & $4.80\pm 0.11$                   & N/A                                   & $84.47\pm 1.49$                  & $7.58\pm 0.06$                   & \multicolumn{1}{r|}{N/A}              & $98.65\pm 0.03$                  & $6.35\pm 0.10$                   & \multicolumn{1}{r|}{N/A}              & $72.13\pm 0.07$                  & $7.18\pm 0.08$                   & \multicolumn{1}{r|}{N/A}              & $58.57\pm 0.04$                  & $6.50\pm 0.77$                   & N/A                                  \\ \midrule
% \textbf{CF-$k$}                                       & $18.60\pm 2.30$                  & $92.88\pm 0.51$                  & \multicolumn{1}{r|}{$89.05\pm 0.93$}  & $7.71\pm 0.18$                   & $33.61\pm 0.93$                  & \multicolumn{1}{r|}{$30.76\pm 0.86$}  & $16.03\pm 0.09$                  & $36.67\pm 1.98$                  & $33.14\pm 0.74$                       & $18.60\pm 2.30$                  & $9.65\pm 0.15$                   & \multicolumn{1}{r|}{$7.70\pm 0.27$}   & $15.22\pm 0.05$                  & $9.58\pm 0.09$                   & \multicolumn{1}{r|}{$7.57\pm 0.05$}   & $48.17\pm 1.76$                  & $9.30\pm 0.12$                   & \multicolumn{1}{r|}{$7.37\pm 0.06$}   & $16.41\pm 0.73$                  & $9.49\pm 0.15$                   & $6.79\pm 0.06$                       \\
% \textbf{EF-$k$}                                       & $31.77\pm 1.56$                  & $15.34\pm 0.01$                  & \multicolumn{1}{r|}{$14.05\pm 0.17$}  & $17.59\pm 3.31$                  & $8.80\pm 0.08$                   & \multicolumn{1}{r|}{$7.84\pm 0.24$}   & $21.66\pm 0.70$                  & $8.92\pm 0.77$                   & $7.10\pm 0.10$                        & $20.08\pm 1.35$                  & $9.03\pm 0.23$                   & \multicolumn{1}{r|}{$7.38\pm 0.06$}   & $17.96\pm 1.54$                  & $9.4\pm 0.21$                    & \multicolumn{1}{r|}{$7.16\pm 0.05$}   & $52.18\pm 0.53$                  & $9.03\pm 0.06$                   & \multicolumn{1}{r|}{$6.92\pm 0.05$}   & $16.41\pm 1.33$                  & $9.39\pm 0.04$                   & $6.85\pm 0.85$                       \\
% \textbf{L1-Sparse}                                    & $91.84\pm 0.55$                  & $22.17\pm 0.14$                  & \multicolumn{1}{r|}{$17.87\pm 0.42$}  & $94.16\pm 0.06$                  & $23.24\pm 0.59$                  & \multicolumn{1}{r|}{$17.25\pm 0.22$}  & $95.42\pm 0.01$                  & $22.23\pm 0.05$                  & $16.83\pm 0.13$                       & $75.78\pm 1.48$                  & $16.20\pm 0.24$                  & \multicolumn{1}{r|}{$13.77\pm 0.46$}  & $59.01\pm 1.67$                  & $8.61\pm 0.09$                   & \multicolumn{1}{r|}{$5.66\pm 0.09$}   & $67.26\pm 0.19$                  & $16.27\pm 0.73$                  & \multicolumn{1}{r|}{$14.14\pm 0.59$}  & $82.30\pm 1.96$                  & $15.95\pm 0.02$                  & $12.36\pm 0.32$                      \\ \midrule
% \textbf{EWC}                                          & $90.93\pm 0.46$                  & $7.18\pm 0.08$                   & \multicolumn{1}{r|}{$5.10\pm 0.01$}   & $82.78\pm 1.02$                  & $9.34\pm 0.08$                   & \multicolumn{1}{r|}{$5.91\pm 0.04$}   & $92.70\pm 0.81$                  & $9.35\pm 0.04$                   & $6.03\pm 0.04$                        & $76.24\pm 2.14$                  & $9.64\pm 0.05$                   & \multicolumn{1}{r|}{$6.69\pm 0.03$}   & $74.14\pm 0.78$                  & $9.06\pm 0.22$                   & \multicolumn{1}{r|}{$6.44\pm 0.08$}   & $55.70\pm 2.57$                  & $9.32\pm 0.07$                   & \multicolumn{1}{r|}{$6.77\pm 0.04$}   & $46.51\pm 0.57$                  & $9.19\pm 0.04$                   & $6.56\pm 0.01$                       \\
% \textbf{CDC}                                          &                                  &                                  & \multicolumn{1}{r|}{}                 &                                  &                                  & \multicolumn{1}{r|}{}                 &                                  &                                  &                                       &                                  &                                  & \multicolumn{1}{r|}{}                 &                                  &                                  & \multicolumn{1}{r|}{}                 &                                  &                                  & \multicolumn{1}{r|}{}                 &                                  &                                  &                                      \\
% \textbf{RSSA}                                         & $38.36\pm 0.09$                  & $12.70\pm 0.17$                  & \multicolumn{1}{r|}{$13.54\pm 0.40$}  & $71.96\pm 0.21$                  & $25.41\pm 0.06$                  & \multicolumn{1}{r|}{$19.08\pm 0.59$}  & $79.54\pm 0.32$                  & $34.59\pm 0.26$                  & $25.33\pm 0.39$                       & $32.07\pm 0.58$                  & $17.79\pm 0.02$                  & \multicolumn{1}{r|}{$15.99\pm 0.08$}  & $22.70\pm 1.47$                  & $18.83\pm 0.08$                  & \multicolumn{1}{r|}{$14.87\pm 0.16$}  & $31.70\pm 1.89$                  & $20.35\pm 0.34$                  & \multicolumn{1}{r|}{$18.63\pm 0.01$}  & $26.21\pm 0.17$                  & $22.24\pm 0.16$                  & $18.09\pm 0.02$                      \\ \midrule
% \textbf{Retraining}                                   & $98.80\pm 0.09$                  & $4.94\pm 0.04$                   & \multicolumn{1}{r|}{N/A}              & $98.58\pm 0.28$                  & $5.24\pm 0.09$                   & \multicolumn{1}{r|}{N/A}              & $99.72\pm 0.01$                  & $4.80\pm 0.11$                   & N/A                                   & $84.47\pm 1.49$                  & $7.58\pm 0.06$                   & \multicolumn{1}{r|}{N/A}              & $98.65\pm 0.03$                  & $6.35\pm 0.10$                   & \multicolumn{1}{r|}{N/A}              & $72.13\pm 0.07$                  & $7.18\pm 0.08$                   & \multicolumn{1}{r|}{N/A}              & $58.57\pm 0.04$                  & $6.50\pm 0.77$                   & N/A                                  \\
% \textbf{Extrapolation}                                & $95.10\pm 0.69$                  & $41.39\pm 1.76$                  & \multicolumn{1}{r|}{$42.98\pm 0.68$}  & $94.50\pm 0.05$                  & $17.90\pm 0.35$                  & \multicolumn{1}{r|}{$27.81\pm 0.37$}  & $90.90\pm 0.12$                  & $45.79\pm 0.29$                  & $44.30\pm 0.40$                       & $89.54\pm 0.09$                  & $11.54\pm 0.07$                  & \multicolumn{1}{r|}{$11.02\pm 0.06$}  & $94.35\pm 0.12$                  & $12.18\pm 0.04$                  & \multicolumn{1}{r|}{$10.12\pm 0.07$}  & $94.44\pm 0.34$                  & $23.44\pm 0.02$                  & \multicolumn{1}{r|}{$26.40\pm 0.30$}  & $92.80\pm 0.14$                  & $23.70\pm 0.07$                  & $19.10\pm 0.10$                      \\
% \textbf{NL2}                                          & $97.85\pm 2.25$                  & $9.69\pm 0.07$                   & \multicolumn{1}{r|}{$6.70\pm 0.25$}   & $93.03\pm 0.70$                  & $10.50\pm 0.34$                  & \multicolumn{1}{r|}{$6.26\pm 0.12$}   & $97.92\pm 0.67$                  & $9.95\pm 0.17$                   & $6.70\pm 0.18$                        & $90.41\pm 0.19$                  & $11.92\pm 0.46$                  & \multicolumn{1}{r|}{$8.69\pm 0.05$}   & $93.99\pm 1.70$                  & $9.60\pm 0.25$                   & \multicolumn{1}{r|}{$6.44\pm 0.11$}   & $97.13\pm 1.42$                  & $14.70\pm 0.55$                  & \multicolumn{1}{r|}{$9.03\pm 0.13$}   & $83.76\pm 3.21$                  & $12.81\pm 0.88$                  & $7.93\pm 0.99$                       \\
% \textbf{IL2}                                          & $92.97\pm 0.48$                  & $13.06\pm 0.46$                  & \multicolumn{1}{r|}{$16.55\pm 0.54$}  & $90.39\pm 1.36$                  & $15.54\pm 0.05$                  & \multicolumn{1}{r|}{$8.64\pm 0.90$}   & $98.28\pm 0.55$                  & $9.72\pm 0.31$                   & $11.64\pm 0.46$                       & $84.05\pm 1.03$                  & $13.09\pm 0.10$                  & \multicolumn{1}{r|}{$9.07\pm 0.18$}   & $94.00\pm 0.75$                  & $11.31\pm 0.06$                  & \multicolumn{1}{r|}{$7.25\pm 0.13$}   & $83.51\pm 2.18$                  & $12.94\pm 0.89$                  & \multicolumn{1}{r|}{$9.87\pm 0.04$}   & $75.23\pm 6.25$                  & $13.12\pm 0.78$                  & $6.11\pm 0.24$                       \\
% \textbf{EL2}                                          & $99.32\pm 0.43$                  & $9.65\pm 0.21$                   & \multicolumn{1}{r|}{$6.29\pm 0.18$}   & $96.23\pm 0.54$                  & $10.24\pm 0.19$                  & \multicolumn{1}{r|}{$5.80\pm 0.04$}   & $95.22\pm 0.34$                  & $8.89\pm 0.52$                   & $5.68\pm 0.10$                        & $90.45\pm 1.02$                  & $11.16\pm 0.08$                  & \multicolumn{1}{r|}{$7.94\pm 0.32$}   & $94.40\pm 2.19$                  & $9.45\pm 0.96$                   & \multicolumn{1}{r|}{$6.31\pm 0.64$}   & $93.97\pm 2.65$                  & $11.07\pm 0.86$                  & \multicolumn{1}{r|}{$7.83\pm 0.05$}   & $93.63\pm 0.42$                  & $9.66\pm 0.58$                   & $9.84\pm 0.23$                       \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}


% \begin{table}[!t]
%     \caption{PUL ($\uparrow$), FID ($\downarrow$) and Ret-FID ($\downarrow$) after unlearning MNIST classes. FID of pre-trained GAN: $5.4$.}
%     \centering
%     \resizebox{0.43\textwidth}{!}{
%         \begin{tabular}{cc|ccc|cccc|c|ccc}
%             \toprule
%             \textbf{Features} & \textbf{Metrics} & \textbf{CFK} & \textbf{EFK} & \textbf{L1-Sparse} & \textbf{EWC} & \textbf{CDC} & \textbf{RSSA} & \textbf{Retraining} & \textbf{Extrapolation} & \textbf{$\gL_{repulsion}^{\text{NL2}}$} & \textbf{$\gL_{repulsion}^{\text{IL2}}$} & \textbf{$\gL_{repulsion}^{\text{EL2}}$} \\ \midrule

%             \multirow{3}{*}{\textbf{Class-1}} & PUL & 3.60 $\pm$ 0.18 & 31.77 $\pm$ 1.56 & 91.84 $\pm$ 0.55 & 90.93 $\pm$ 0.46 &  &  & 98.80 $\pm$ 0.90 & 95.10 $\pm$ 0.69 & 97.85 $\pm$ 2.25 & 92.97 $\pm$ 0.48 & \textbf{99.32 $\pm$ 0.43} \\ 
%             & FID & 92.88 $\pm$ 0.51 & 15.34 $\pm$ 0.10 & 27.17 $\pm$ 0.14 & 7.18 $\pm$ 0.08 &  &  & 4.94 $\pm$ 0.04 & 41.39 $\pm$ 1.76 & 9.69 $\pm$ 0.07 & 13.06 $\pm$ 0.46 & \textbf{9.65 $\pm$ 0.21}  \\
%             & Ret-FID & & & & & & & & 42.98 $\pm$ 0.68 & 6.70 $\pm$ 0.25 & 16.55  $\pm$ 0.54 & \textbf{6.29 $\pm$ 0.18} \\
%             \midrule
            

%             \multirow{3}{*}{\textbf{Class-4}} & PUL & & & & & & & & 94.50 $\pm$ 0.05 & 93.03 $\pm$ 0.7 & 90.39 $\pm$ 1.36 & \textbf{96.23 $\pm$ 0.54} \\ 
%             & FID & & & & & & & & 17.90 $\pm$ 0.35 & 10.50 $\pm$ 0.34 & 15.54 $\pm$ 0.05 & \textbf{10.24 $\pm$ 0.19} \\ 
%             & Ret-FID & & & & & & & & 27.81 $\pm$ 0.37 & 6.26  $\pm$ 0.12 & 8.64 $\pm$ 0.9 &  \textbf{5.80 $\pm$ 0.04} \\
%             \midrule
            
%             \multirow{3}{*}{\textbf{Class-8}} & PUL & & & & & & & & 90.90 $\pm$ 0.12 & 97.92 $\pm$ 0.677 & \textbf{98.28 $\pm$ 0.55} & 95.22 $\pm$ 0.34 \\ 
%             & FID & & & & & & & & 45.79 $\pm$ 0.29 & 9.95 $\pm$ 0.177 & 9.72 $\pm$ 0.31 & \textbf{8.89 $\pm$ 0.52} \\ 
%             & Ret-FID & & & & & & & & 44.3 $\pm$ 0.40 & 6.70 $\pm$ 0.18 & 11.64 $\pm$ 0.46 & \textbf{5.68  $\pm$ 0.10} \\
%             \bottomrule
            
%         \end{tabular}
%         \label{tab:mnist-unlearning-results}
%     }
% \end{table}

% \begin{table}[!t]
%     \caption{PUL ($\uparrow$), FID ($\downarrow$) and Ret-FID ($\downarrow$) after unlearning CelebA-HQ features. FID of pre-trained GAN: $5.3$.}
%     \centering
%     \resizebox{0.43\textwidth}{!}{
%         \begin{tabular}{cc|ccc|cccc|c|ccc}
%         \toprule
%         \textbf{Features} & \textbf{Metrics} & \textbf{CFK} & \textbf{EFK} & \textbf{L1-Sparse} & \textbf{EWC} & \textbf{CDC} & \textbf{RSSA} & \textbf{Retraining} & \textbf{Extrapolation} & \textbf{$\gL_{repulsion}^{\text{NL2}}$} & \textbf{$\gL_{repulsion}^{\text{IL2}}$} & \textbf{$\gL_{repulsion}^{\text{EL2}}$} \\ \midrule 

%         \multirow{3}{*}{\textbf{Bangs}} & PUL & & & & & & & &  89.54 $\pm$ 0.09 & 90.41 $\pm$ 0.19 & 84.05 $\pm$ 1.03  & \textbf{90.45 $\pm$ 1.02} \\
%         & FID & & & & & & & & 11.54 $\pm$ 0.07 & 11.92 $\pm$ 0.46 & 13.09 $\pm$ 0.10 & \textbf{11.16 $\pm$ 0.08} \\ 
%         & Ret-FID & & & & & & & & 11.02 $\pm$ 0.06 & 08.69 $\pm$ 0.05 & 09.07 $\pm$ 0.18 & \textbf{07.94 $\pm$ 0.32} \\ 
%         \midrule

%         \multirow{3}{*}{\textbf{Hat}} & PUL & & & & & & & & 94.35 $\pm$ 0.12  & 93.99 $\pm$ 1.70 & 94.00 $\pm$ 0.75 & \textbf{94.40 $\pm$ 2.19} \\
%         & FID & & & & & & & & 12.18 $\pm$ 0.04 & 9.60 $\pm$ 0.25 & 11.31 $\pm$ 0.06 & \textbf{9.45 $\pm$ 0.96} \\
%         & Ret-FID & & & & & & & & 10.12 $\pm$ 0.07  & 06.44 $\pm$ 0.11  & 07.25 $\pm$ 0.13 & \textbf{06.31 $\pm$ 0.64} \\ 
%         \midrule

%         \multirow{3}{*}{\textbf{Bald}} & & & & & & & & PUL & 94.44 $\pm$ 0.34          & \textbf{97.13 $\pm$ 1.42} & 83.51 $\pm$ 2.18 & 93.97 $\pm$ 2.65 \\
%         & FID & & & & & & & & 23.44 $\pm$ 0.02 & 14.7 $\pm$ 0.55 & 12.94 $\pm$ 0.89 & \textbf{11.07  $\pm$ 0.86} \\
%         & Ret-FID & & & & & & & & 26.40 $\pm$ 0.30  & 09.03 $\pm$ 0.13  & 09.87 $\pm$ 0.04  & \textbf{07.83 $\pm$0.05}\\ 
%         \midrule

%         \multirow{3}{*}{\textbf{Eyeglasses}} & PUL & & & & & & & & 92.80 $\pm$ 0.14    & 83.76 $\pm$ 3.21 & 75.23 $\pm$ 6.25 & \textbf{93.63 $\pm$ 0.42} \\
%         & FID & & & & & & & & 23.70 $\pm$ 0.07 & 12.81 $\pm$ 0.88 & 13.12 $\pm$ 0.78 & \textbf{9.66 $\pm$ 0.58}  \\
%         & Ret-FID & & & & & & & & 19.10 $\pm$ 0.10  & 07.93 $\pm$ 0.99 & \textbf{06.11 $\pm$ 0.24} & 09.84$\pm$0.23 \\
%         \bottomrule
% \end{tabular}
% \label{tab:celebahq-unlearning-results}}
% \end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}


\begin{table*}[!ht]
\centering
\caption{PUL ($\uparrow$), FID ($\downarrow$) and Ret-FID ($\downarrow$) after unlearning MNIST, AFHQ classes and CelebA-HQ features. }
\label{tab:comb-results}
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{l|ll|r|rrr|rrr|r|rrr}
\toprule
\textbf{Dataset}                     & \textbf{Features}                    & \textbf{Metrics} & \multicolumn{1}{c|}{\textbf{Retraining}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}CF-$k$\\ \citep{goel2022towards}\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}EU-$k$\\ \citep{goel2022towards}\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}$\ell$1-Sparse\\ \citep{jia2023model}\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}EWC\\ \citep{Few_Shot_Generation_EWC}\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}CDC\\ \citep{ojha2021few-shot-gan}\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}RSSA\\ \citep{RSSA}\end{tabular}}} & \multicolumn{1}{c|}{\textbf{Extrapolation}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}$\gL_{repulsion}^{\text{NL2}}$\\(Ours)  \end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}$\gL_{repulsion}^{\text{IL2}}$\\(Ours)  \end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}$\gL_{repulsion}^{\text{EL2}}$\\(Ours)  \end{tabular}}} \\ \midrule
\multirow{9}{*}{\textbf{MNIST}}      & \multirow{3}{*}{\textbf{Class 1}}    & \textbf{PUL}     & $98.80\pm 0.09$                          & $18.60\pm 2.30$                     & $31.77\pm 1.56$                     & $91.84\pm 0.55$                         & $90.93\pm 0.46$                  &                 $90.70\pm 0.16$                 & $38.36\pm 0.09$                    & $95.10\pm 0.69$                             & $97.85\pm 2.25$                  & $92.97\pm 0.48$                  & $\boldsymbol{99.32\pm 0.43}$                  \\
                                     &                                      & \textbf{FID}     & $4.94\pm 0.04$                           & $92.88\pm 0.51$                     & $15.34\pm 0.01$                     & $22.17\pm 0.14$                         & $7.18\pm 0.08$                   &                    $20.85\pm0.49$              & $12.70\pm 0.17$                    & $41.39\pm 1.76$                             & $9.69\pm 0.07$                   & $13.06\pm 0.46$                  & $9.65\pm 0.21$                   \\
                                     &                                      & \textbf{Ret-FID} & N/A                                      & $89.05\pm 0.93$                     & $14.05\pm 0.17$                     & $17.87\pm 0.42$                         & $5.10\pm 0.01$                   &     $17.51\pm1.86$                             & $13.54\pm 0.40$                    & $42.98\pm 0.68$                             & $6.70\pm 0.25$                   & $16.55\pm 0.54$                  & $6.29\pm 0.18$                   \\ \cmidrule{2-14} 
                                     & \multirow{3}{*}{\textbf{Class 4}}    & \textbf{PUL}     & $98.58\pm 0.28$                          & $7.71\pm 0.18$                      & $17.59\pm 3.31$                     & $94.16\pm 0.06$                         & $82.78\pm 1.02$                  &                    $42.39\pm0.66$              & $71.96\pm 0.21$                    & $94.50\pm 0.05$                             & $93.03\pm 0.70$                  & $90.39\pm 1.36$                  & $\boldsymbol{96.23\pm 0.}$                  \\
                                     &                                      & \textbf{FID}     & $5.24\pm 0.09$                           & $33.61\pm 0.93$                     & $8.80\pm 0.08$                      & $23.24\pm 0.59$                         & $9.34\pm 0.08$                   &                      $17.82\pm1.99$            & $25.41\pm 0.06$                    & $17.90\pm 0.35$                             & $10.50\pm 0.34$                  & $15.54\pm 0.05$                  & $10.24\pm 0.19$                  \\
                                     &                                      & \textbf{Ret-FID} & N/A                                      & $30.76\pm 0.86$                     & $7.84\pm 0.24$                      & $17.25\pm 0.22$                         & $5.91\pm 0.04$                   &     $12.39\pm2.32$                             & $19.08\pm 0.59$                    & $27.81\pm 0.37$                             & $6.26\pm 0.12$                   & $8.64\pm 0.90$                   & $5.80\pm 0.04$                   \\ \cmidrule{2-14} 
                                     & \multirow{3}{*}{\textbf{Class 8}}    & \textbf{PUL}     & $99.72\pm 0.01$                          & $16.03\pm 0.09$                     & $21.66\pm 0.70$                     & $95.42\pm 0.01$                         & $92.70\pm 0.81$                  &                         $18.86\pm0.92$         & $79.54\pm 0.32$                    & $90.90\pm 0.12$                             & $97.92\pm 0.67$                  & $\boldsymbol{98.28\pm 0.55}$                  & $95.22\pm 0.34$                  \\
                                     &                                      & \textbf{FID}     & $4.80\pm 0.11$                           & $36.67\pm 1.98$                     & $8.92\pm 0.77$                      & $22.23\pm 0.05$                         & $9.35\pm 0.04$                   &                        $11.18\pm2.28$          & $34.59\pm 0.26$                    & $45.79\pm 0.29$                             & $9.95\pm 0.17$                   & $9.72\pm 0.31$                   & $8.89\pm 0.52$                   \\
                                     &                                      & \textbf{Ret-FID} & N/A                                      & $33.14\pm 0.74$                     & $7.10\pm 0.10$                      & $16.83\pm 0.13$                         & $6.03\pm 0.04$                   &      $12.38\pm3.73$                            & $25.33\pm 0.39$                    & $44.30\pm 0.40$                             & $6.70\pm 0.18$                   & $11.64\pm 0.46$                  & $5.68\pm 0.10$                   \\ \midrule


\multirow{9}{*}{\textbf{AFHQ}}      & \multirow{3}{*}{\textbf{Cat}}    & \textbf{PUL}     & $93.37\pm0.23$                          & $15.74\pm0.41$                     & $16.08\pm0.28$                     & $86.25\pm 1.35$                         & $90.58\pm1.54$                  &                 $28.57\pm0.43$                 & $66.86\pm0.22$                    & $90.64\pm0.33$                             & $94.28\pm 0.17$                  & $90.93\pm0.51$                  & $\boldsymbol{95.76\pm0.25}$                  \\
                                     &                                      & \textbf{FID}     & $12.45\pm0.16$                           & $42.91\pm0.33$                     & $43.21\pm0.25$                     & $25.73\pm0.05$                         & $15.30\pm0.98$                   &                    $59.76\pm0.40$              & $59.88\pm0.35$                    & $45.89\pm2.60$                             & $16.29\pm 0.06$                   & $20.69\pm0.04$                  & $16.50\pm0.12$                   \\
                                     &                                      & \textbf{Ret-FID} & N/A                                      & $37.34\pm0.29$                     & $37.62\pm0.42$                     & $14.96\pm0.11$                         & $8.29\pm0.04$                   &     $49.93\pm1.02$                             & $46.80\pm0.62$                    & $38.87\pm1.93$                             & $8.93\pm1.23$                   & $9.86\pm0.08$                  & $8.17\pm0.14$                   \\ \cmidrule{2-14} 
                                     & \multirow{3}{*}{\textbf{Dog}}    & \textbf{PUL}     & $85.96\pm0.21$                          & $13.12\pm0.12$                      & $10.30\pm0.13$                     & $68.21\pm0.15$                         & $68.79\pm0.08$                  &                    $9.60\pm0.24$              & $54.54\pm0.36$                    & $82.08\pm1.02$                             & $75.33\pm0.35$                  & $76.53\pm0.51$                  & $\boldsymbol{79.21\pm0.18}$                  \\
                                     &                                      & \textbf{FID}     & $5.71\pm0.43$                           & $64.50\pm0.58$                     & $32.69\pm0.23$                      & $19.54\pm0.53$                         & $10.38\pm1.08$                   &                      $47.85\pm0.53$            & $55.06\pm0.20$                    & $25.54\pm1.19$                             & $8.62\pm0.08$                  & $9.37\pm1.06$                  & $9.31\pm0.14$                  \\
                                     &                                      & \textbf{Ret-FID} & N/A                                      & $65.72\pm2.31$                     & $31.40\pm0.36$                      & $15.10\pm0.85$                         & $8.50\pm0.35$                   &     $46.79\pm0.67$                             & $53.24\pm0.34$                    & $24.98\pm1.35$                             & $5.96\pm0.45$                   & $6.84\pm0.10$                   & $7.13\pm0.12$                   \\ \cmidrule{2-14} 
                                     & \multirow{3}{*}{\textbf{Wild}}    & \textbf{PUL}     & $88.60\pm0.22$                          & $16.40\pm0.55$                     & $16.63\pm0.84$                     & $84.05\pm0.45$                         & $73.44\pm0.16$                  &                         $6.51\pm0.13$         & $43.99\pm0.72$                    & $84.45\pm0.11$                             & $82.82\pm0.77$                  & $80.96\pm0.18$                  & $\boldsymbol{89.09\pm0.25}$                  \\
                                     &                                      & \textbf{FID}     & $15.24\pm0.24$                           & $35.56\pm0.11$                     & $35.80\pm0.39$                      & $37.63\pm0.52$                         & $16.32\pm0.08$                   &                        $42.17\pm0.19$          & $60.95\pm0.45$                    & $45.98\pm2.66$                             & $17.69\pm0.18$                   & $22.70\pm0.11$                   & $19.67\pm0.69$                   \\
                                     &                                      & \textbf{Ret-FID} & N/A                                      & $34.47\pm0.94$                     & $32.55\pm0.14$                      & $21.80\pm0.16$                         & $14.38\pm0.01$                   &      $36.95\pm0.28$                            & $44.20\pm0.32$                    & $41.86\pm1.99$                             & $14.89\pm0.13$                   & $13.76\pm0.12$                  & $14.90\pm0.65$                   \\ \midrule



\multirow{12}{*}{\textbf{CelebA-HQ}} & \multirow{3}{*}{\textbf{Bangs}}      & \textbf{PUL}     & $84.47\pm 1.49$                          & $18.60\pm 2.30$                     & $20.08\pm 1.35$                     & $75.78\pm 1.48$                         & $76.24\pm 2.14$                  &  $83.76\pm0.12$                                & $32.07\pm 0.58$                    & $89.54\pm 0.09$                             & $90.41\pm 0.19$                  & $84.05\pm 1.03$                  & $\boldsymbol{90.45\pm 1.02}$                 \\
                                     &                                      & \textbf{FID}     & $7.58\pm 0.06$                           & $9.65\pm 0.15$                      & $9.03\pm 0.23$                      & $16.20\pm 0.24$                         & $9.64\pm 0.05$                   &                  $34.66\pm1.94$                & $17.79\pm 0.02$                    & $11.54\pm 0.07$                             & $11.92\pm 0.46$                  & $13.09\pm 0.10$                  & $11.16\pm 0.08$                  \\
                                     &                                      & \textbf{Ret-FID} & N/A                                      & $7.70\pm 0.27$                      & $7.38\pm 0.06$                      & $13.77\pm 0.46$                         & $6.69\pm 0.03$                   &                      $24.67\pm0.02$            & $15.99\pm 0.08$                    & $11.02\pm 0.06$                             & $8.69\pm 0.05$                   & $9.07\pm 0.18$                   & $7.94\pm 0.32$                   \\ \cmidrule{2-14} 
                                     & \multirow{3}{*}{\textbf{Hat}}        & \textbf{PUL}     & $98.65\pm 0.03$                          & $15.22\pm 0.05$                     & $17.96\pm 1.54$                     & $59.01\pm 1.67$                         & $74.14\pm 0.78$                  &                    $85.23\pm0.77$              & $22.70\pm 1.47$                    & $94.35\pm 0.12$                             & $93.99\pm 1.70$                  & $94.00\pm 0.75$                  & $\boldsymbol{94.40\pm 2.19}$                  \\
                                     &                                      & \textbf{FID}     & $6.35\pm 0.10$                           & $9.58\pm 0.09$                      & $9.4\pm 0.21$                       & $8.61\pm 0.09$                          & $9.06\pm 0.22$                   &                       $23.48\pm0.12$           & $18.83\pm 0.08$                    & $12.18\pm 0.04$                             & $9.60\pm 0.25$                   & $11.31\pm 0.06$                  & $9.45\pm 0.96$                   \\
                                     &                                      & \textbf{Ret-FID} & N/A                                      & $7.57\pm 0.05$                      & $7.16\pm 0.05$                      & $5.66\pm 0.09$                          & $6.44\pm 0.08$                   &                        $17.46\pm0.22$          & $14.87\pm 0.16$                    & $10.12\pm 0.07$                             & $6.44\pm 0.11$                   & $7.25\pm 0.13$                   & $6.31\pm 0.64$                   \\ \cmidrule{2-14} 
                                     & \multirow{3}{*}{\textbf{Bald}}       & \textbf{PUL}     & $72.13\pm 0.07$                          & $48.17\pm 1.76$                     & $52.18\pm 0.53$                     & $67.26\pm 0.19$                         & $55.70\pm 2.57$                  &                 $90.10\pm0.37$                & $31.70\pm 1.89$                    & $94.44\pm 0.34$                             & $\boldsymbol{97.13\pm 1.42}$                  & $83.51\pm 2.18$                  & $93.97\pm 2.65$                  \\
                                     &                                      & \textbf{FID}     & $7.18\pm 0.08$                           & $9.30\pm 0.12$                      & $9.03\pm 0.06$                      & $16.27\pm 0.73$                         & $9.32\pm 0.07$                   &                      $26.96\pm0.02$            & $20.35\pm 0.34$                    & $23.44\pm 0.02$                             & $14.70\pm 0.55$                  & $12.94\pm 0.89$                  & $11.07\pm 0.86$                  \\
                                     &                                      & \textbf{Ret-FID} & N/A                                      & $7.37\pm 0.06$                      & $6.92\pm 0.05$                      & $14.14\pm 0.59$                         & $6.77\pm 0.04$                   &                   
                                     $17.99\pm0.09$               & $18.63\pm 0.01$                    & $26.40\pm 0.30$                             & $9.03\pm 0.13$                   & $9.87\pm 0.04$                   & $7.83\pm 0.05$                   \\ \cmidrule{2-14} 
                                     & \multirow{3}{*}{\textbf{Eyeglasses}} & \textbf{PUL}     & $58.57\pm 0.04$                          & $16.41\pm 0.73$                     & $16.41\pm 1.33$                     & $82.30\pm 1.96$                         & $46.51\pm 0.57$                  &                $91.65\pm0.31$                  & $26.21\pm 0.17$                    & $92.80\pm 0.14$                             & $83.76\pm 3.21$                  & $75.23\pm 6.25$                  & $\boldsymbol{93.63\pm 0.42}$                  \\
                                     &                                      & \textbf{FID}     & $6.50\pm 0.77$                           & $9.49\pm 0.15$                      & $9.39\pm 0.04$                      & $15.95\pm 0.02$                         & $9.19\pm 0.04$                   &                    $36.66\pm0.02$              & $22.24\pm 0.16$                    & $23.70\pm 0.07$                             & $12.81\pm 0.88$                  & $13.12\pm 0.78$                  & $9.66\pm 0.58$                   \\
                                     &                                      & \textbf{Ret-FID} & N/A                                      & $6.79\pm 0.06$                      & $6.85\pm 0.85$                      & $12.36\pm 0.32$                         & $6.56\pm 0.01$                   &                         $30.08\pm0.27$         & $18.09\pm 0.02$                    & $19.10\pm 0.10$                             & $7.93\pm 0.99$                   & $6.11\pm 0.24$                   & $9.84\pm 0.23$                   \\ \bottomrule
\end{tabular}%
}
\end{table*}
% \vspace{-5mm}
